Understanding the Impact of UGC Specificities on Translation Quality

This work takes a critical look at the evaluation of user-generated content automatic translation, the well-known specificities of which raise many challenges for MT. Our analyses show that measuring the average-case performance using a standard metric on a UGC test set falls far short of giving a reliable image of the UGC translation quality. That is why we introduce a new data set for the evaluation of UGC translation in which UGC specificities have been manually annotated using a fine-grained typology. Using this data set, we conduct several experiments to measure the impact of different kinds of UGC specificities on translation quality, more precisely than previously possible.

==> Intro_djame.tex <==
%-*- coding: utf-8 -*-
\section{Introduction \label{sec:intro}}

Neural Machine Translation (NMT) models fall far short from being able
to translate noisy User-Generated Content (UGC): the quality of their
translation is often even worse than that of a traditional
phrase-based
system~\cite{DBLP:conf/aclnmt/KhayrallahK18,rosales-nunez-etal-2019-comparison}.
In addition to ambiguous grammatical constructs and the profusion of
ellipsis, the main difficulty encountered when translating UGC is the
high number of out-of-vocabulary tokens (OOVs) resulting from
misspelled words, emoticons, hashtags, mentions and all specific
constructs used in online forums and social medias
\cite{foster-2010-cba,seddah-etal-2012-french,eisenstein-2013-bad}.
Some of those phenomena can be perceived as noise while the others
are typical markers of language variations among speakers.  More over,
a certain amount of those same phenomena operate at the character or
at the subword levels, hence the natural question of finding the right
neural architecture and its ideal level of representation to model
both noise and language variation is of crucial importance.

This is why, focusing on the noise axis, we present in this work a
thorough evaluation of three out-of-the-box NMT architectures applied
to noisy UGC in a zero-shot scenario. \textcolor{red}{To understand
  the impact of UGC idiosyncrasies on translation quality and better
  understand how these idiosyncrasies are handled by various neural
  architecture,} we provide a framework that enables us to generate a
collection of annotated parallel corpora with a dynamic controllable
number of UGC idiosyncrasies \textcolor{red}{and noise types} per
sentence. \textcolor{red}{Thanks to our approach, we are able to
  highlight the `atomic' challenges raised by each type of UGC as well
  as the potential complex latent dynamics between difféerent UGC
  specificities.}
  
% Our approach allow us to control the noise types which are present at
% evaluation time by retaining only a subset of the noise occurrences,
% such that the impact on performance can be assessed by removing
% potentially complex latent dynamics between different UGC
% specificities. Those can lead to the intractability of
% individual\draftnote{atomic?} challenges raised by such types of UGC
% idiosyncrasies for NMT.\draftnote{Ce paragraphe est vraiment dur à
%   comprendre, on dirait qu'il est circulaire -ds}


Our results show that ... \fbox{todo}.
By analyzing and comparing errors
  made by our different systems (char-based NMT, Seq2seq and
  Transformer-based NMT) using our typology and data, we
  illustrate the usefulness of our annotated collection, as we show
evidence that (i) char-based neural machine translation models are
extremely sensitive to unknown and rare characters, (ii) we noticed
advantages over BPE-based models when translating misspelled words,
incorrect tokenization and inconsistent casing and (iii) by
drastically limiting their vocabulary size, we can improve their
generalization ability when facing noisy text.\draftnote{a revoir, on
  dirait qu'on vend des cacahuettes, c'est relou -ds} 


% \iffalse  
% %%% C'est relou José, on dirait que tu vends des charM







% .....
% to
% explain and characterize challenges posed by these kind of texts, such
% that upcoming works can easily evaluate and develop MT systems that
% are more robust to real-world noise. 

% \draftremove{In order to illustrate our
% approach, we choose to investigate the impact of UGC noise on
% different subword levels.}



% In this regard, char-based models appear to offer a
% natural solution to this
% problem~\cite{luong16achieving,ling15character}: indeed these open
% vocabulary models are designed specifically to address the OOV
% problem. This is why, as part of our comparison, we make use of out-of-the-box character-based
% NMT models \cite{DBLP:journals/tacl/LeeCH17_et_al} to potentially address a range of
% challenges raised by UGC translation. While character-based models may
% seem promising for such task, to the best of our knowledge, they have
% only been tested on either data sets in which noise has been
% artificially added %through sampling an edited word error data set
% \cite{DBLP:conf/iclr/BelinkovB18, ebrahimi18adversarial} or
% canonical data sets, in which they prove to be very effective for
% translating morphologically rich languages with a high number of OOV
% \cite{luong16achieving}.

% However our experiments (\textsection \ref{sec:exp}) show that
% character-based systems are globally outperformed by Byte-pair
% Encoding (BPE) models when translating noisy UGC. \textcolor{red}{In
%   order to understand this counter-intuitive result and derive
%   insights beyond a coarse corpus-level metric, we present our
%   evaluation framework to quantify the impact of noise on translation
%   quality as our main contribution, by including a new data set of
%   noisy UGC in which UGC peculiarities have been manually annotated
%   with their position using a fine-grained typology.% {Mettre plus
%   % l'accent sur le data set si on soumet sur la track Lang Resource and
%   % Evaluation -ds}


% \draftremove{Our contributions can be seen as a negative result as we
% show that character-based NMT models are unable to cope with an ever
% evolving domain with an endless productivity of out-of-vocabulary
% characters.}

% \fi

==> Makefile <==
# set latexfile to the name of the main file without the .tex

latexfile = acl2021

#latexfile = ANR_ParSiTi
# put the names of figure files here.  include the .eps
figures = 
includedfiles = Intro_djame.tex
    
TEX = pdflatex

# *.fig files may be in ./Figs
vpath %.fig Figs

$(latexfile).dvi : $(figures) $(includedfiles) $(latexfile).tex


%.eps : %.fig
	fig2dev -L eps $< > $@

$(latexfile).pdf : $(latexfile).tex $(includedfiles)
	${TEX} $(latexfile).tex $(latexfile).pdf

pdf :	$(latexfile).pdf
	#ps2pdf $(latexfile).ps $(latexfile).pdf
	${TEX} $(latexfile).tex $(latexfile).pdf

bib :	$(latexfile).dvi
	bibtex $(latexfile)
	${TEX} $(latexfile)
	${TEX} $(latexfile)
	bibtex $(latexfile)
	${TEX} $(latexfile)
	${TEX} $(latexfile) 

$(latexfile).ps : $(latexfile).dvi
	dvips  -t a4 -Ppdf $(latexfile) -o $(latexfile).ps

ps : $(latexfile).ps 

$(latexfile).tar.gz : $(figures) $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $(figures) $(latexfile).tex Figs/*.fig

tarball: $(latexfile).tar.gz


clean: 
	rm -f $(latexfile).bbl
	rm -f $(latexfile).log
	rm -f $(latexfile).dvi
	rm -f $(latexfile).blg
	rm -f $(latexfile).aux
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf
check:
	cat $(latexfile).log | grep undef
count:
	wc -c Objectifs.tex Retombes.tex resume.en.tex resume.fr.tex Programme.tex

dist-clean: clean
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf

view: $(latexfile).pdf
	open -a Skim.app $(latexfile).pdf

preview: $(latexfile).pdf
	open -a Preview.app $(latexfile).pdf


edit:
	xemacs $(latexfile).tex 2> /dev/null &

countLREC: pdf
	pdf2ps $(latexfile).pdf $(latexfile).ps 
	ps2ascii $(latexfile).ps | /usr/bin/wc -w

commit_svn:
	svn commit -m "(minor) up" ./

up:
	git pull

commit:
	git commit -m "update" ./
	git push
		
	

progress:
	thesis_progress.sh $(latexfile).pdf 45

ipad: 
	cp $(latexfile).pdf /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/=HDR/$(latexfile)_$(shell gdate +%F_%R).pdf
	open /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/=HDR/
	
	
papers:
	cp -v -R -n ./papers_hdr/ /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/=HDR/
	open /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/=HDR/
	         
	
	

==> old/Intro_djame.tex <==
%-*- coding: utf-8 -*-
\section{Introduction  (used for the be arxived paper don't use here)\label{sec:intro}}

Neural Machine Translation (NMT) models fall far short from being able
to translate noisy User-Generated Content (UGC): the quality of their
translation is often even worse than that of a traditional
phrase-based
system~\cite{DBLP:conf/aclnmt/KhayrallahK18,rosales-nunez-etal-2019-comparison}.
In addition to ambiguous grammatical constructs and the profusion of
ellipsis, the main difficulty encountered when translating UGC is the
high number of out-of-vocabulary tokens (OOVs) resulting from
misspelled words, emoticons, hashtags, mentions and all specific
constructs used in online forums and social mediahttps://www.overleaf.com/projects
\cite{foster-2010-cba,seddah-etal-2012-french,eisenstein-2013-bad}.
Some of those phenomena can be perceived as noise while the others
are typical markers of language variations among speakers.  More over,
a certain amount of those same phenomena operate at the character or
at the subword levels, hence the natural question of finding the right
neural architecture and its ideal level of representation to model
both noise and language variation is of crucial importance.

This is why, focusing more on the noise axis, we present in this work
a thorough evaluation of three out-of-the-box NMT architectures
(namely \chartchar, \seqtseq and \transformer) applied to noisy UGC in
a zero-shot scenario. To understand the impact of UGC idiosyncrasies
on translation quality and better understand how these idiosyncrasies
are handled by various neural architecture, we have manually annotated
a parallel corpus of UGC to indicate the position and type of each UGC
idiosyncrasy. We introduced a framework that enables us to generate a
collection of annotated parallel corpora with a dynamic controllable
number of UGC idiosyncrasies and noise types per sentence. Thanks to
our approach, we are able to highlight the `atomic' challenges raised
by each type of UGC as well as the potential complex latent dynamics
between difféerent UGC specificities. While, we focus, in this work,
on machine translation, We believe that the annotated corpus and the
framework we present could be of great interest to perform
fine-grained error analysis for NLP systems dealing with noisy UGC.
  
% Our approach allow us to control the noise types which are present at
% evaluation time by retaining only a subset of the noise occurrences,
% such that the impact on performance can be assessed by removing
% potentially complex latent dynamics between different UGC
% specificities. Those can lead to the intractability of
% individual\draftnote{atomic?} challenges raised by such types of UGC
% idiosyncrasies for NMT.\draftnote{Ce paragraphe est vraiment dur à
%   comprendre, on dirait qu'il est circulaire -ds}


By analyzing and comparing errors made by our different systems using
our typology and data, we illustrate the usefulness of our annotated
collection, as we show evidence that (i) char-based neural machine
translation models are extremely sensitive to unknown and rare
characters, (ii) we noticed advantages over BPE-based models when
translating misspelled words, incorrect tokenization and inconsistent
casing and (iii) by drastically limiting their vocabulary size, we can
improve their generalization ability when facing noisy
text.\draftnote{a revoir, on dirait qu'on vend des cacahuettes, c'est
  relou -ds}


% \iffalse  
% %%% C'est relou José, on dirait que tu vends des charM







% .....
% to
% explain and characterize challenges posed by these kind of texts, such
% that upcoming works can easily evaluate and develop MT systems that
% are more robust to real-world noise. 

% \draftremove{In order to illustrate our
% approach, we choose to investigate the impact of UGC noise on
% different subword levels.}



% In this regard, char-based models appear to offer a
% natural solution to this
% problem~\cite{luong16achieving,ling15character}: indeed these open
% vocabulary models are designed specifically to address the OOV
% problem. This is why, as part of our comparison, we make use of out-of-the-box character-based
% NMT models \cite{DBLP:journals/tacl/LeeCH17_et_al} to potentially address a range of
% challenges raised by UGC translation. While character-based models may
% seem promising for such task, to the best of our knowledge, they have
% only been tested on either data sets in which noise has been
% artificially added %through sampling an edited word error data set
% \cite{DBLP:conf/iclr/BelinkovB18, ebrahimi18adversarial} or
% canonical data sets, in which they prove to be very effective for
% translating morphologically rich languages with a high number of OOV
% \cite{luong16achieving}.

% However our experiments (\textsection \ref{sec:exp}) show that
% character-based systems are globally outperformed by Byte-pair
% Encoding (BPE) models when translating noisy UGC. \textcolor{red}{In
%   order to understand this counter-intuitive result and derive
%   insights beyond a coarse corpus-level metric, we present our
%   evaluation framework to quantify the impact of noise on translation
%   quality as our main contribution, by including a new data set of
%   noisy UGC in which UGC peculiarities have been manually annotated
%   with their position using a fine-grained typology.% {Mettre plus
%   % l'accent sur le data set si on soumet sur la track Lang Resource and
%   % Evaluation -ds}


% \draftremove{Our contributions can be seen as a negative result as we
% show that character-based NMT models are unable to cope with an ever
% evolving domain with an endless productivity of out-of-vocabulary
% characters.}

% \fi

==> old/related_work.tex <==
\section{Character-level NMT: a solution to cope with noisy text?  \label{sec:rw}}

% \textcolor{red}{GW: pour moi ce paragraphe est redondant avec l'intro}
% We intend to use character-level NMT approaches to investigate to what
% extent they can cope with UGC specificities. Character-based systems
% seem promising in this setup since they are, by design,
% open-vocabulary and can therefore model the inner semantics of
% potential OOV words \newcite{DBLP:conf/acl/ChungCB16_et_al}.

In this work, we explore two character-based translation models.  The
first model we consider, \texttt{charCNN}, is a classic encoder-decoder
in which the encoder uses character-based embeddings in combination
with convolutional and highway layers to replace the standard look-up
based word representations. % The model considers, as input, a stream of
% words (i.e. it assumes the input has been tokenized beforehand) and
% tries to learn a word representation that is more robust to noise by
% unveiling regularities at the character level, however, predictions
% are made at the word level. 
This architecture was initially proposed
by~\newcite{DBLP:conf/aaai/KimJSR16} for language modeling;
\newcite{DBLP:conf/acl/Costa-JussaF16} show how it can be used in a
NMT system. Improvements up to +3 \textsc{Bleu} points are reported on
the standard German-English WMT task.

The second model we employ does not rely on an explicit segmentation:
\newcite{DBLP:journals/tacl/LeeCH17_et_al} introduce a the \chartchar
model that directly maps a source characters sequence to a target
characters sequence without any segmentation thanks to a
character-level convolutional network with stride max-pooling at the
encoder.  \newcite{DBLP:journals/tacl/LeeCH17_et_al} show that this
model outperforms subword-level translation models on several WMT
tasks.

These two models have been originally tested on WMT tasks (i.e. texts
that mostly qualify as canonical with very few spelling or grammatical
errors). The impact of noise on \texttt{charCNN} has been evaluated by
\newcite{DBLP:conf/iclr/BelinkovB18} and
\newcite{DBLP:conf/coling/EbrahimiLD18} by adding noise to canonical
text (the \texttt{TEDTalk} dataset). Their results show that both
\texttt{charCNN} and \chartchar fail to translate even moderately
noisy texts when only trained on `clean' data \textcolor{red}{GW: et
  quand on ajoute des données noisy en apprentissage}. More recently,
\newcite{DBLP:journals/corr/abs-1911-04997_et_al} showed, in the same
setting, that character-based Transformer is more robust that its
BPE-based counterparts when trained on `clean' data and tested on high
`natural noise', although this difference disappears when noisy
samples are used to augment the training dataset.

All these works consider `noisy' corpora built by sampling Wikipedia
edits % XXX ref to wicopaco dans la version finale
and therefore consider that noise mainly results from typographical
and spelling errors. To the best of our knowledge, no work has studied
the performance of character-based models have never been tested on
`ecological' noisy data such as the one that can be found in UGC. This
sets the main motivation for this work, \textcolor{red}{specially through
  proposing new evaluation methods and resources for such kind of
  texts.}

\textcolor{red}{GW: et la typologie d'erreur que djamé avait trouvée
  ?}
  
% \section{Related Work: Noisy UGC MT Evaluation \label{sec:rw}}
\textcolor{red}{On the other hand, evaluation of MT performance on noisy UGC is also
challenging as it is difficult to identify precise caveats to overcome
beyond coarse metrics such as BLEU scores on noisy corpora at test
time. Adequacy and fluency have been also been widely used as
translation metrics \cite{DBLP:conf/amta/WhiteOO94}, often facilitated
by manual inspection of the predictions, which may differ from
automated metrics' results
\cite{DBLP:journals/pbml/CastilhoMGCTW17}. In terms of approach, a
related work to this study is that of
\cite{DBLP:conf/coling/FujiiMAHMSI20}, who proposed a quantitative
analysis on UGC test partitions by annotating Name Entities (NE),
abbreviations, colloquial expressions and lexical variants in Ja-Fr
noisy UGC translation. Perhaps the closest work to ours on UGC
evaluation is \cite{DBLP:conf/acl/NiuMDA20}, also performing a study
on performance impact for the case-changing and misspellings comparing
subword-level and subword regularization NMT on 4 languages
pairs. Both of these studies are focused in the MTNT UGC corpus and
including 4SQ for the latter. In this same line of research, we intend
to expand/continue these efforts for characterizing noisy UGC impact
on NMT by providing insights on a extensive and fine-grained list of
documented UGC peculiarities in a fairly new Fr-En UGC corpus. By
making available such collection of text and data augmentation
framework, we aspire to encourage future research identifying and
tracking advancements of new MT models aiming to produce MT models
more robust to this kind on texts.}

